OThink-R1: Intrinsic Fast/Slow Thinking Mode Switching for Over-Reasoning Mitigation

Human cognition operates through two complementary modes: fast intuitive thinking and slow deliberate thinking. Vanilla large language models (LLMs) predominantly follow the fast-thinking paradigm, producing immediate responses; while recent large reasoning models (LRMs) adopt slow-thinking strategies, generating detailed reasoning chains before arriving at answers. While LRMs often achieve higher accuracy, this comes at the cost of substantially increased token usage. To address this efficiency-accuracy trade-off, we propose OThink-R1, a hybrid reasoning framework that integrates both modes within a single LRM and enables automatic mode switching based on problem characteristics. We first identify three major patterns of essential and redundant reasoning trajectories in LRMs, which guide the design of an auxiliary LLM-based judge that adaptively determines when slow thinking is necessary. Leveraging the judge's decisions, we construct a hybrid fine-tuning dataset by pruning redundant reasoning to produce fast-thinking samples and retaining complete reasoning for slow-thinking samples. This dataset is then used to fine-tune LRMs, equipping them with inherent autonomous mode-selection capabilities. Extensive experiments on mathematical and question-answering benchmarks show that OThink-R1 reduces reasoning token usage significantly while maintaining competitive accuracy. The code is available at https://github.com/AgenticIR-Lab/OThink-R1.

==> tables/LLMJudgePrompt.tex <==

% \begin{promptbox}[System Prompt for Redundant Reasoning Judge]{lightgreen2}{prompt:selection}

% \begin{promptbox}[System Prompt]{lightgreen2}{label:sys-prompt-selection}  % 标题自动显示 "Prompt 1"

% Please act as a classifier for the following task.

% \textbf{Task Overview}: You will receive a question along with its correct answer. The model's thought process will be provided within <think></think> tags. Your job is to evaluate whether the model's thinking is necessary and classify it accordingly.

% \textbf{Criteria for Classification}:

% \textbf{Invalid Thinking}:
%  When the model has already derived the correct answer but continues to think, classify as follows:
%  \begin{enumerate}[leftmargin = *,label=\arabic*)]
%     \item \textbf{Trying Multiple Solutions}: The model has already derived the correct answer. However, the model continue to explore alternative solutions, using phrases like "Is there any chance" or "Another Way."
%     \item \textbf{Repeated Validation}: The model has already derived the correct answer. However, the model continue to check or validates its previous reasoning multiple times.
%     \item \textbf{Invalid Assumptions}: The model has already derived the correct answer.  However, the model continue to propose irrelevant assumptions or scenarios or excessively analyzes details to confirm the correctness of its answer.
% \end{enumerate}


% \textbf{Valid Thinking}:
% Valid thinking can be classified as follows:
% \begin{enumerate}[leftmargin = *,label=\arabic*)]
% \item \textbf{Brief Analysis}: The model provides concise analysis that helps quickly identify the core elements of the problem.
% \item \textbf{Avoiding Ambiguity}: The model ensures a clear understanding of the problem, eliminating potential ambiguities for accurate reasoning.
% \item \textbf{Avoiding Omission of Premises}: The model confirms all necessary premises during the reasoning process to ensure completeness and accuracy.
% \end{enumerate}

% \textbf{Response Format}:
% \begin{enumerate}[leftmargin=*, ,label=-]
%     \item Correct answer: (The correct answer of the question)
%     \item  Is the model's thinking essential or redundant? (yes/no)
%     \item If valid, the reason is? 
%     \item  If invalid, the reason is?
%     \item Thinking category:  <answer> (Valid/Invalid) </answer>`
%     \item Classification:  <subset> class of the response </subset> 
% \end{enumerate}

% Please analyze the model's thought process based on these criteria.
% \end{promptbox}

\begin{promptbox}[System Prompt]{lightgreen2}{label:sys-prompt-selection}

Please act as a classifier for the following task.

\textbf{Task Overview}: You will receive a question along with its correct answer. The model's thought process will be provided within <think></think> tags. Your job is to evaluate whether the model's thinking is necessary and classify it accordingly.

\textbf{Criteria for Classification}:

\textbf{Redundant reasoning}:
When the model has already derived the correct answer but continues to think, classify as follows:
\begin{enumerate}[leftmargin = *,label=\arabic*)]
    \item \textbf{Multi-Solution Exploration}: The model has already derived the correct answer. However, the model continues to explore alternative solutions, using phrases like "Is there any chance" or "Another Way."
    \item \textbf{Repeated Self-Validation}: The model has already derived the correct answer. However, the model continues to check or validates its previous intermediate reasoning steps for several times.
    \item \textbf{Defensive Assumptions}: The model has already derived the correct answer.  However, the model is overly cautious, continuing to propose extraneous hypotheses to confirm the correctness of its answer, which is irrelevant to problem-solving. 
\end{enumerate}


\textbf{Essential Thinking}:
The essential reasoning follows the following principles:
\begin{enumerate}[leftmargin = *,label=\arabic*)]
\item \textbf{Key-word Identification}: The model provides concise analysis that helps quickly identify the key words, core elements of the problem.
\item \textbf{Misunderstanding Prevention}: The model conducts reasoning which aims to eliminate misunderstandings within the problem statement, thereby preventing errors stemming from incorrect assumptions.
\item \textbf{Premise Omission Avoidance}: The model conducts reasoning which confirms all necessary premises of problems to ensure understanding completeness.
\end{enumerate}

\textbf{Response Format}:
\begin{enumerate}[leftmargin=*, ,label=-]
    \item Correct answer: (The correct answer of the question)
    \item  Is the model's thinking essential or redundant? (yes/no)
    \item If essential, the reason is? 
    \item  If redundant, the reason is?
    \item Thinking category: <answer> (Redundant/Essential) </answer>
    \item Classification: <subset> class of the response </subset>
\end{enumerate}

Please analyze the model's thought process based on these criteria.
\end{promptbox}

==> tables/case_question.tex <==


\begin{figure*}[htbp]
\centering
\footnotesize

\modelcomparison{%
    I am providing a question with multiple choices. The answer is one of the choices listed in the choices. Please answer the correct one.
    
    \noindent
    Question:  The man was going fishing instead of work, what is he seeking?
    
    \noindent
    Choices: 
    A. food \quad
    \ans{B. relaxation} \quad
    C. killing \quad
    D. missing morning cartoons \quad
    E. boredom
}{
<think>
\begin{quote}
% ``Okay, so I have this question here: 'The man was going fishing instead of work, what is he seeking?'...''

% % \vspace{0.3cm}
% ``Let me go through the options one by one:

% A. Food – That's about getting food, but fishing is about catching fish. So I don't think this is it.

% B. Relaxation – Relaxation is about being calm or mentally relaxed. If he's fishing, maybe he's feeling Inspired or Determined\ldots''

% \vspace{0.3cm}
``\ldots perhaps the best fit is that \ans{he's seeking relaxation} because fishing provides some form of mental or emotional satisfaction\ldots''

% \vspace{0.3cm}
``\ldots perhaps \ans{he's seeking the relaxation} that comes with fishing.''

% \vspace{0.3cm}
``\ldots the best fit might be that \ans{he's seeking relaxation} because he's enjoying his fishing trip, which could provide that mental or emotional satisfaction, leading him to feel relaxed.''

% \vspace{0.3cm}
``I'm leaning towards E. Boredom because if he's going fishing and it's not fulfilling for him, he might feel bored\ldots''

% \vspace{0.3cm}
``Wait, \ans{maybe the answer is B}. Relaxation because fishing provides that kind of mental release or excitement. But I'm not entirely sure.''

% \vspace{0.3cm}
``I think I'm overcomplicating this.''

% \vspace{0.3cm}
``Alternatively, \ans{maybe the answer is B}. Relaxation because he's doing something else to relax. But I'm not sure.''

% \vspace{0.3cm}
``Wait, maybe the answer is E. Boredom because if he's fishing and he's not bored, he wouldn't go fishing\ldots''

% \vspace{0.3cm}
``I'm going to go with E. Boredom because he's probably not bored unless he's doing something not listed here.''

\end{quote}
</think>


% \vspace{0.5cm}


      \noindent\textbf{E. Boredom}

    
          \noindent\textbf{Step-by-Step Explanation:}
          
          \begin{enumerate}[label=\textbf{\arabic*.}, leftmargin=*, align=left]
    \item \textbf{Understanding the Context}: The man is fishing instead of working, indicating a shift from a job to a hobby. The question asks what he is seeking.

    \item \textbf{Evaluating Choices}:
    \begin{itemize}[label=--]
        \item \textbf{A. Food}: Relates to getting food, not about his activity.
        \item \textbf{B. Relaxation}: Potential, but the question implies he's doing fishing, not resting.
        \item \textbf{C. Killing}: Not relevant.
        \item \textbf{D. Missing morning cartoons}: Seems unrelated.
        \item \textbf{E. Boredom}: If he's not bored, he wouldn't go fishing. Thus, he must be seeking an engaging activity.
    \end{itemize}
\end{enumerate}

\ans{\textbf{Answer: E. Boredom}}
}{%
% \vspace{10pt}
    <think></think>

      The question is asking what the man is seeking when he chooses to go fishing instead of work. The options are food, relaxation, killing, missing morning cartoons, or boredom. Given that he's taking a break from work to go fishing, the most direct consequence is that \ans{he's seeking relaxation}. Going fishing can provide a peaceful and relaxed environment, which might explain his choice.

    Other options like food or boredom could be related to the activity itself but are less direct consequences of his decision. Relaxation is the most fitting answer because it's the core consequence of taking a break from work to engage in an enjoyable activity.
    
    \ans{ANSWER: B}
}

\caption{An example of the switching between fast and slow thinking modes demonstrated on DeepSeek-R1-Distill-Qwen-7B.}
\label{fig:case-study-over-thinking}
\end{figure*}

